Point absorbers in Advanced LIGO

Small, highly absorbing points are randomly present on the surfaces of the main interferometer optics in Advanced LIGO. The resulting nano-meter scale thermo-elastic deformations and substrate lenses from these micron-scale absorbers significantly reduces the sensitivity of the interferometer directly though a reduction in the power-recycling gain and indirect interactions with the feedback control system. We review the expected surface deformation from point absorbers and provide a pedagogical description of the impact on power build-up in second generation gravitational wave detectors (dual-recycled Fabry-Perot Michelson interferometers). This analysis predicts that the power-dependent reduction in interferometer performance will significantly degrade maximum stored power by up to 50% and hence, limit GW sensitivity, but suggests system wide corrections that can be implemented in current and future GW detectors. This is particularly pressing given that future GW detectors call for an order of magnitude more stored power than currently used in Advanced LIGO in Observing Run 3. We briefly review strategies to mitigate the effects of point absorbers in current and future GW wave detectors to maximize the success of these enterprises.

==> CO2.tex <==
\label{sec:CO2}

The CO2 laser projector was installed to provide the ability to apply essentially arbitrary spatially varying wavefront compensation. This is achieved by varying the intensity profile of the applied CO2 laser beam with different masks.


\subsection{Central heating}

The central heating mask was an elliptical aperture that presented a circular hole XXmm in diameter when placed at an angle of approximately 22.5$^\circ$ to the beam. This was then imaged onto the compensation plate with a magnification of $21\times$.

The thermal lens from the CO2 central heating was measured with the HWS. The wavefront distortion is shown in Figure \ref{fig:HWS_CO2}.

\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{figures/CO2_laser_HWS_wavefront_map.png}
  \caption{Measurement of CO2 thermal lens using HWS [LHO 14736]. In this instance, the center of the HWS beam is translated approximately [\SI{-50}{\milli\meter}, \SI{+25}{\milli\meter}] relative to the center of the CO2 heating profile. The circular pattern outside the }
\label{fig:HWS_CO2}
\end{figure} 

\subsection{Interferometer response}

\subsubsection{Contrast defect}

\subsubsection{Power recycling}


\subsection{Annular heating}
\tcr{Check for annular heating measurements}.

The wavefront distortion from annular heating has yet to be measured. As the input power has been limited to approximately 20\% of full power, this is yet to be required in interferometer operations. The annular compensation is not expected to be required before full power operation, expected in O4 \cite{ObservingScenarios2018}.

CO2 results
- intensity noise coupling measurements

- DARM response

- Effect on contrast defect

- HWS measurements. Spatial and transient response

- effect on IFO performance?

- annular heating





\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{figures/CO2_defocus_measurement.png}
  \caption{Measurement of CO2 thermal lens using HWS at LLO [aLOG 27334].}
\label{fig:HWS_CO2_defocus}
\end{figure} 







==> CouplingOfRIN.tex <==

\begin{figure}[h]
  \centering
  \includegraphics[width=\columnwidth]{figures/RIN_coupling.png}
  \caption{MIST model of elevated RIN coupling with different positions of point absorbers}
  \label{fig:RIN_coupling}
  % Figure 1 from P1500260
\end{figure}


\begin{itemize}
    \item Sideband effects (ITM thermal lens)
    \item Prediction of IFO going forwawrd without PA mitigation. Evan note on reduced build up with excess losses in the arms
\end{itemize}



==> HOM_model.tex <==
HOM model goes here

==> IFOPerformancePredictions.tex <==

\Aidan{- power and intensity noise coupling? Or just include these in the earlier plots and discuss them here?}

% \begin{figure}[h]
%   \centering
%   \includegraphics[width=\columnwidth]{figures/arm_power_v_input_power.png}
%   \caption{Hiro model of arm power vs input power projecting out significantly reduced stored power as we increase input power}
%   \label{fig:arm_power_v_input_power}
%   % Figure 1 from P1500260
% \end{figure}


==> PAmitigation.tex <==
\label{sec:mitigation}

Appropriated mitigation of point absorbers will requires (a) elimination, where possible, of the introduction of absorbing material into the coatings and (b) implementation of some form of multi-element front surface heater to provide adaptive correction of surface deformations in the interferometer. 

\subsection{Elimination of absorbing material}

Attempts to clean the material off of coatings has been unsuccessful. Possible alternatives include micro-machining the absorbing area, i.e drilling out a region of order \SI{100}{\micro\meter} in diameter to eliminate point absorbers in the optics.

Alternatively, if the source of the absorbing particles originates as part of the coating process, a  diagnostic and adjustment of that process may yield a solution.

\subsection{Front-surface multi-element heater}

Several different designs for a multi-element front surface heater have been proposed over recent years. Any such device will have some strict requirements on it in order to significantly reduce scattering into HOM whilst not introducing apparent displacement noise into the interferometer.

There is resonant enhancement of the losses of a subset of the possible HOMs. As such, a multi-element heater design that targets these modes has the potential to be significantly more efficient than one that simply has a brute-force approach of many square heater pixels. This is an active area of research and specific engineering designs are still to be established. Nevertheless, any actuator will have to meet the following requirements in order to interface with the interferometer optics.

\begin{enumerate}
    \item Relative Intensity Noise: Any intensity noise fluctuations in the heating beam will induce  deformations in the surface of the optic. This was demonstrated by Ballmer \cite{BallmerThesis}. The exact requirements will depend on the spatial intensity distribution of the heating beam, however, as a guide, a beam with a Gaussian weighted average power of \SI{1}{\watt} will require a RIN of less than $10^{-9}$ at \SI{20}{\hertz}  in order to not couple displacement noise in the interferometer.
    \item Total Power
    \item Number of pixels
\end{enumerate}

{\it List the requirements in the LVC talk.}

\begin{itemize}
    \item Replacement of optics
    \item Requirements for a front-surface heater
    \item Losses from very high spatial frequencies are not recoverable
    \item Resonant losses from intermediate spatial frequencies are recoverable.
    \item plot the cavity linewidth for higher order modes in the cavity - to show the losses vs HOM number
\end{itemize}

% \begin{figure}
%   \centering
%   \includegraphics[width=\columnwidth]{figures/surface_deform.png}
%   \caption{Example surface deformation from LHO}
%   \label{fig:surface_deformation}
%   % Figure 1 from P1500260
% \end{figure}

% \begin{figure}
%   \centering
%   \includegraphics[width=\columnwidth]{figures/surface_correction.png}
%   \caption{Example surface correction from LHO}
%   \label{fig:surface_deformation}
%   % Figure 1 from P1500260
% \end{figure}


==> PRGvBeamPosition.tex <==
\label{s:IFOrealign}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/RTLvPosn.pdf}
    \caption{The round-trip loss (RTL) as a function of position for a point absorber that absorbs \SI{10}{\milli\watt} of power independent of position (blue) and the RTL for a point absorber where \SI{10}{\milli\watt} is absorbed in the center of the interferometer beam on the ETM and the absorption is then scaled by the position dependent intensity of the interferometer (red). \Aidan{Get this actual data from Hiro}.}
    \label{fig:RTL_v_posn}
\end{figure}

The SIS models of arm cavity loss and PRG reduction in the presence of point absorbers show a strong  dependence of the loss on the position of that point absorber relative to the center of the interferometer beam. This is illustrated in Figure \ref{fig:RTL_v_posn}. For a point that absorbs \SI{10}{\milli\watt} regardless of position (i.e. has constant surface deformation), the blue curve shows the round-trip loss as a function of absorber position. This is useful in analyzing the case where a HWS measurement is made and the absorbed power is calculated to be \SI{10}{\milli\watt} but there is some uncertainty in the location of that point relative to the interferometer beam.


\begin{itemize}
    \item Modeling (SIS) shows that PRG loss is strongly dependent on point absorber position
    \item A factor of two (or more) reduction in loss is predicted from model. \Aidan{Do we have a model where the reduction includes the lowered point absorber magnitude}. The explanation for this is given by Hiro.
    \item This was observed in interferometer (LLO) when the \Aidan{beams} were steered to different positions on the test masses. Recovered a lot of PRG: compare the pre- and post-realign plots in Figure \ref{fig:PRG_v_power}.
    \item Also saw the measured arm power increase \ref{fig:BS_power}.
    \item Point absorbers on ETMX and ETMY were reduced in size
    \item LLO Arm results showing the PRG decreases vs input power and reflectivity decrease vs input power
\end{itemize}



%\subsubsection{With beam position}

Moving the beam position dramatically increased the build-up.





==> RH.tex <==
\label{sec:RH}

The ring heaters (RH) in Advanced LIGO are coaxial with the ITMs and ETMs based upon the design developed by Zhao et al. \cite{PhysRevLett.96.231101}. They radiate thermal energy on the barrels of these test masses to simultaneously create controllable surface deformation and thermo-refractive lenses in the substrates.

\subsection{Surface curvature measurements - cavity scan}

The higher-order mode spacing in the Fabry-Perot arms is dependent on the cavity g-factor which is, in turn, dependent on the surface curvature of the test masses. As a result, the effect of ring heater on the surface curvature of the test mass was determined by locking one arm of the interferometer and measuring the deviation of the higher-order mode spacing as function of time as the RH was applied to the ETM.

The 4-km FP arm was scanned to measure the frequency response of the cavity. Several higher order spatial modes were located in this cavity scan. The frequency of these modes was measured to measure the cavity g-factor (and the ETM HR surface RoC). 

The ETM RH was applied at 13.3W to measure the change in the higher order mode spacing as a function of time. The results were compared to the COMSOL model described in the previous section and are illustrated in Figure \ref{fig:RH_ROC_cavity_scan}. These results show that the measured change in the RoC is approximately 29\% larger than the predicted change in the RoC.


\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{figures/RH_cavity_scan.pdf}
  \caption{Measurement of RH surface curvature via tracking of HOM frequency. The RH was turned on with 13.3W output power at time $t=0$. A simple finite-element model of the thermal system was created. It agrees to within approximately 6\%. As the time scale of the measurement increases, the exact nature of the boundary conditions becomes more important and the accuracy of  a simple model is expected to decrease. The cavity-scan technique demonstrates occasional glitches in the data which are visible as data points lying well outside one standard deviation.}
\label{fig:RH_ROC_cavity_scan}
\end{figure} 

\subsection{HWS measurements of RH thermal lens}

\subsubsection{HWS-measured wavefront distortion - 2D}
%https://alog.ligo-la.caltech.edu/aLOG/index.php?callRep=34263
% This covers the command line plotting tool

The spatial response of the ring heater was measured with the Hartmann sensor. The wavefront distortion was highly axially symmetric and contained a strong spherical power term producing a single-pass thermal lens of \SI{-9}{\micro\diopter}/W. The gradient field and wavefront distortion at time $t\approx\,$\SI{7750}{\second} are shown in Figures \ref{fig:HWS_RH} and \ref{fig:HWS_RH}, respectively. The residual wavefront distortion, once the spherical power component has been subtracted, is shown in Figure \ref{fig:HWS_RH}. The RMS value of this is \SI{12345}{\nano\meter}.

\tcr{Can be thought of as two exponentials - one corresponds to heat flowing into the center. The other's rate is determined by the time constant for radiation to the environment.}

\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{figures/RH_laser_HWS_wavefront_map.png}
  \caption{Measurement of ring heater thermal lens with HWS at LLO [LLO aLOG 36595].}
\label{fig:HWS_RH}
\end{figure} 


\subsubsection{HWS measurement of transient response of RH-induced thermal lens}

To characterize the ring heater, we applied a step function to the ring heater power and determined the resulting response by measuring the spherical power (thermal lensing) with the HWS. The results are shown in Figure \ref{fig:HWS_RH_TL_defocus}. At time t=0, the RH power was set to 4W output power. The resulting single-pass thermal lens was measured with the HWS for approximately 36 hours.

Also shown is a fit to the data using the equation:
\begin{equation}
S_{RH} = dS/dP_{SS}\,\Delta P\, \left(-1 + \sum_{i=1}^{3}\, a_{i}\,\exp\left(\frac{-t}{\tau_{i}} \right)\right)
\end{equation}

\noindent where $\Delta P$ is the change in power and the parameters $dS/dP_{SS} = -9.0$\SI{}{\micro\diopter}/W, $a_{i}$ and $\tau_{i}$ are presented in Table \ref{tab:RH_params}. This response can be modeled in IIR filter bank as the sum of three poles:

\begin{equation}
dS/dP_{SS}\, \left(\sum_{i=1}^{3}\, a_{i}\,f_{i}\right)
\end{equation}

\noindent where $f_{i} = 1/\left(2\,\pi\, \tau_{i}\right)$ and $\sum_{i=1}^{3} a_{i} = 1$. These pole values are also listed in Table \ref{tab:RH_params}.

% see LLO alOG 25656
\begin{table}[h!]
  \begin{center}
    \caption{Ring heater step function parameter fit. \tcr{check this as amplitudes don't sum to 1}}
    \label{tab:RH_params}
    \begin{tabular}{|c|c|c|c|} % <-- Changed to S here.
    \hline
      \textbf{Index} & \textbf{Amp.} & \textbf{Time const. (s)} & \textbf{Pole freq. (\SI{}{\micro\hertz})}\\
      \hline
      $i$ & $a_{i}$ & $\tau_{i}$ &  $f_{i}$\\
      \hline
      1 & -6.06 & 1600 & 99.7 \\
      2 & 8.53 & 2450 & 65.1\\
      3 & -1.47 & 28600 & 5.57  \\
      \hline
    \end{tabular}
  \end{center}
\end{table}

% 


\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{figures/RH_TL_time_evolution.pdf}
%  \caption{Measurement of RH thermal lens at LLO [LHO aLOG 26030, LLO aLOG 15213].}
  \caption{Measurement of RH thermal lens at LLO. The COMSOL mode of the lens included an efficiency factor of 78\% that was determined by Ramette et al. \cite{Ramette:16}.}
\label{fig:HWS_RH_TL_defocus}
\end{figure} 


A thermal model of the test masses was presented by Wang et al. \cite{Wang:2017_Thermal_model}.

\subsection{RH temperature monitor}
 The RH contains a PT100 RTD temperature sensor that is built into the lower ring heater segment shield. This sensor monitors the temperature of the aluminum shield. The interior surface of the aluminum shield is gold coated. The response of this temperature sensor is shown in Figure \ref{fig:RH_temperature}. 
 
The change in temperature of the ring heater itself is determined by measuring the change in the resistance of the nichrome wire. 

This demonstrates that the majority ($>$X\%) of the energy is radiated onto the test mass. Determine the surface area of the outer part of the shield and assume that this is radiating (what about the thermal conduction)? \tcr{Use a log-log plot and $\Delta$T}.


\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{figures/LLO_RH_Step_8349_temperature.pdf}
  \caption{Measurement of RH RTD temperature at LLO [aLOG 8349].}
\label{fig:RH_temperature}
\end{figure} 

\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{figures/RH_resistivity_temperature.pdf}
  \caption{Measurement of RH temperature calculated from the change in resistivity of the nichrome (Chromel-C) wire at LHO when 26W is applied to the RH. The red curve is an exponential fit used to estimate the effective time constant of the ring heater power. The yellow and purple curves are derived from finite-element models of the RH in which \SI{26}{W} and \SI{20.3}{\watt} (= \SI{26}{W} $\times 78\%$) of power, respectively, is dissipated in the RH substrate. [aLOG 3863].}
\label{fig:RH_temp_self}
\end{figure} 




==> auth_only_file.tex <==
\author[1,*]{Aidan F. Brooks} 
\author[1]{Gabriele Vajente} 
\author[1]{Hiro Yamamoto} 
\author[1]{Rich Abbott} 
\author[2]{Carl Adams} 
\author[1]{Rana X. Adhikari} 
\author[1]{Alena Ananyeva} 
\author[1]{Stephen Appert} 
\author[1]{Koji Arai} 
\author[3]{Joseph S. Areeda} 
\author[4]{Yasmeen Asali} 
\author[2]{Stuart M. Aston} 
\author[5]{Corey Austin} 
\author[6]{Anne M. Baer} 
\author[7]{Matthew Ball} 
\author[8]{Stefan W. Ballmer} 
\author[9]{Sharan Banagiri} 
\author[10]{David Barker} 
\author[11]{Lisa Barsotti} 
\author[10]{Jeffrey Bartlett} 
\author[12]{Beverly K. Berger} 
\author[2]{Joseph Betzwieser} 
\author[13]{Dripta Bhattacharjee} 
\author[1]{Garilynn Billingsley} 
\author[11,1]{Sebastien Biscans} 
\author[2]{Carl D. Blair} 
\author[10]{Ryan M. Blair} 
\author[14,15]{Nina Bode} 
\author[14,15]{Phillip Booker} 
\author[1]{Rolf Bork} 
\author[2]{Alyssa Bramley} 
\author[16]{Daniel D. Brown} 
\author[11]{Aaron Buikema} 
\author[1]{Craig Cahillane} 
\author[17]{Kipp C. Cannon} 
\author[16]{Huy Tuong Cao}
\author[18]{Xu Chen} 
\author[16]{Alexei A. Ciobanu} 
\author[10]{Filiberto Clara} 
\author[10]{Camilla Compton} 
\author[19]{Sam J. Cooper} 
\author[4]{Kenneth R. Corley} 
\author[4]{Stefan T. Countryman} 
\author[20]{Pep B. Covas} 
\author[1]{Dennis C. Coyne} 
\author[21]{Laurence E. Datrier} 
\author[8]{Derek Davis} 
\author[19]{Chiara D. Difronzo} 
\author[22,23]{Katherine L. Dooley} 
\author[10]{Jenne C. Driggers} 
\author[21]{Peter Dupej} 
\author[10]{Sheila E. Dwyer} 
\author[2]{Anamaria Effler} 
\author[1]{Todd Etzel} 
\author[11]{Matthew Evans} 
\author[2]{Tom M. Evans} 
\author[1]{Jon Feicht} 
\author[11]{Alvaro Fernandez-Galiana} 
\author[11]{Peter Fritschel} 
\author[2]{Valery V. Frolov} 
\author[24]{Paul Fulda} 
\author[2]{Michael Fyffe} 
\author[5,2]{Joe A. Giaime} 
\author[2]{Dwayne D. Giardina} 
\author[25]{Patrick Godwin} 
\author[5,13,38]{Evan Goetz} 
\author[11]{Slawomir Gras} 
\author[10]{Corey Gray} 
\author[21]{Rachel Gray} 
\author[24]{Anna C. Green}
\author[1]{Anchal Gupta}
\author[1]{Eric K. Gustafson} 
\author[26]{Dick Gustafson} 
\author[11]{Evan Hall}
\author[10]{Jonathan Hanks} 
\author[2]{Joe Hanson} 
\author[5]{Terra Hardwick} 
\author[2]{Raine K. Hasskew} 
\author[2]{Matthew C. Heintze} 
\author[7]{Adrian F. Helmling-Cornell} 
\author[27]{Nathan A. Holland} 
\author[10]{Jeff D. Jones} 
\author[28]{Shivaraj Kandhasamy} 
\author[7]{Sudarshan Karki} 
\author[1]{Marie Kasprzack} 
\author[10]{Keita Kawabe} 
\author[27]{Nutsinee Kijbunchoo} 
\author[10]{Peter J. King} 
\author[10]{Jeffrey S. Kissel} 
\author[10]{Rahul Kumar} 
\author[10]{Michael Landry} 
\author[11]{Benjamin B. Lane} 
\author[12]{Brian Lantz} 
\author[2]{Michael Laxen} 
\author[10]{Yannick K. Lecoeuche} 
\author[26]{Jessica Leviton} 
\author[14  15]{Liu Jian} 
\author[2]{Marc Lormand} 
\author[29]{Andrew P. Lundgren} 
\author[22]{Ronaldas Macas} 
\author[11]{Myron Macinnis} 
\author[22]{Duncan M. Macleod} 
\author[10,11]{Georgia L. Mansell} 
\author[4]{Szabolcs Marka} 
\author[4]{Zsuzsanna Marka} 
\author[19]{Denis V. Martynov} 
\author[11]{Ken Mason} 
\author[11]{Thomas J. Massinger} 
\author[1,11]{Fabrice Matichard} 
\author[11]{Nergis Mavalvala} 
\author[10]{Richard McCarthy} 
\author[27]{David E. McClelland} 
\author[2]{Scott McCormick} 
\author[11]{Lee McCuller} 
\author[1,38]{Jessica McIver} 
\author[27]{Terry McRae} 
\author[10]{Gregory Mendell} 
\author[7]{Kara Merfeld} 
\author[10]{Edmond L. Merilh} 
\author[14,15]{Fabian Meylahn} 
\author[30]{Timesh Mistry} 
\author[11]{Richard Mittleman} 
\author[10]{Gerardo Moreno} 
\author[19]{Conor M. Mow-Lowry} 
\author[29]{Simone Mozzon} 
\author[2]{Adam Mullavey} 
\author[2]{Timothy J. Nelson} 
\author[7]{Philippe Nguyen} 
\author[29]{Laura K. Nuttall} 
\author[10]{Jason Oberling} 
\author[2]{Richard J. Oram} 
\author[1]{Charles Osthelder} 
\author[16]{David J. Ottaway} 
\author[2]{Harry Overmier} 
\author[7]{Jordan R. Palamos} 
\author[2,31]{William Parker} 
\author[32]{Ethan Payne} 
\author[2]{Arnaud Pele} 
\author[26]{Reilly Penhorwood} 
\author[10]{Carlos J. Perez} 
\author[10]{Marc Pirello} 
\author[10]{Hugh Radkins} 
\author[33]{Karla E. Ramirez} 
\author[1]{Jonathan W. Richardson} 
\author[26]{Keith Riles} 
\author[1,21]{Norna A. Robertson} 
\author[1]{Jameson G. Rollins} 
\author[10]{Chandra L. Romel} 
\author[2]{Janeen H. Romie} 
\author[34]{Michael P. Ross} 
\author[10]{Kyle Ryan} 
\author[10]{Travis Sadecki} 
\author[1]{Eduardo J. Sanchez} 
\author[1]{Luis E. Sanchez} 
\author[28]{Saravanan R. Tiruppatturrajamanikkam} 
\author[10]{Richard L. Savage} 
\author[1]{Dean Schaetzl} 
\author[35]{Roman Schnabel} 
\author[7]{Robert M. Schofield} 
\author[2]{Eyal Schwartz} 
\author[2]{Danny Sellers} 
\author[10]{Thomas Shaffer} 
\author[10]{Daniel Sigg} 
\author[27]{Bram J. Slagmolen} 
\author[3]{Joshua R. Smith} 
\author[5]{Siddharth Soni} 
\author[21]{Borja Sorazu} 
\author[21]{Andrew P. Spencer} 
\author[21]{Ken A. Strain} 
\author[1]{Ling Sun} 
\author[24]{Marek J. Szczepanczyk} 
\author[2]{Michael Thomas} 
\author[10]{Patrick Thomas} 
\author[2]{Keith A. Thorne} 
\author[21]{Karl Toland} 
\author[1]{Calum I. Torrie} 
\author[2]{Gary Traylor} 
\author[11]{Maggie Tse} 
\author[5]{Alexander L. Urban} 
\author[5]{Guillermo Valdes} 
\author[8]{Daniel C. Vander-Hyde} 
\author[16]{Peter J. Veitch} 
\author[34]{Krishna Venkateswara} 
\author[1]{Gautam Venugopalan} 
\author[36]{Aaron D. Viets} 
\author[8]{Thomas Vo} 
\author[10]{Cheryl Vorvick} 
\author[37]{Madeline Wade} 
\author[27]{Robert L. Ward} 
\author[10]{Jim Warner} 
\author[10]{Betsy Weaver} 
\author[11]{Rainer Weiss} 
\author[11]{Chris Whittle} 
\author[15,14]{Benno Willke} 
\author[1]{Christopher C. Wipf} 
\author[1]{Liting Xiao} 
\author[11]{Hang Yu} 
\author[11]{Haocun Yu} 
\author[1]{Liyuan Zhang} 
\author[11,1]{Michael E. Zucker} 
\author[1]{John Zweizig} 


==> fitting.tex <==

\textcolor{red}{Fit point absorbers using first couple of minutes of data. Fit uniform absorption using later data. Do I fit points first and then subtract them off or do I use a routine that encompasses all the times? How do i weight the early data more? Maybe just use a logarithm set of times steps of data. Also, use r = 3.5mm as the point absorber size.}

==> measurements.tex <==
\label{sec:measurements}
% \begin{figure}[h]
%   \centering
%   \includegraphics[width=\columnwidth]{figures/Self_Heating_PointAbs_HWS_wavefront_map.png}
%   \caption{H1 ITMX point absorber as measured by the Hartmann wavefront sensor during O2. This was the first point absorber discovered in Advanced LIGO. This optic was replaced after O2.}
%   \label{fig:H1ITMX}
%   % Figure 1 from P1500260
% \end{figure}


\begin{figure}[h]
  \centering
  \includegraphics[width=\columnwidth]{figures/H1-ITMX_1180229513_1180229634.pdf}
  \caption{H1 ITMX point absorber as measured by the Hartmann wavefront sensor during O2, approximately 120s after power-up. (GPS times of HWS measurements: $t_{\mathrm{REF}} = 1180229513$ [May 31, 2017 01:31:35 UTC], $t_{\mathrm{LIVE}} = 1180229634$).}
  \label{fig:H1ITMXa}
  % Figure 1 from P1500260
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=\columnwidth]{figures/H1-ITMX_1180229513_1180232835.pdf}
  \caption{H1 ITMX point absorber as measured by the Hartmann wavefront sensor during O2, approximately 55 minutes after power-up. (GPS times of HWS measurements: $t_{\mathrm{REF}} = 1180229513$ [May 31, 2017 01:31:35 UTC], $t_{\mathrm{LIVE}} = 1180232835$).}
  \label{fig:H1ITMXb}
  % Figure 1 from P1500260
\end{figure}


\begin{figure}[h]
  \centering
%  \includegraphics[width=\columnwidth]{figures/Self_Heating_Uniform_HWS_wavefront_map.png}
  \includegraphics[width=\columnwidth]{figures/L1-ITMY_1176677676_1176679964.pdf}
  \caption{Example of uniform absorption. L1 ITMY during O2. This image is consistent with XX uniform absorption. (GPS times of HWS measurements: $t_{\mathrm{REF}} = 1176677676$ [April 19, 2017 22:54:18 UTC], $t_{\mathrm{LIVE}} = 1176679964$).}
  \label{fig:L1ITMX}
  % Figure 1 from P1500260
\end{figure}



In this section we describe HWS measurements of the individual test masses installed in Advanced LIGO in O2 and O3. Of the eight optics measured, point absorbers were found on five of those optics.

\textcolor{red}{Maybe quote the residual RMS after point absorber fit has been removed (and uniform absorption fit). This gives a measure of the uncertainty/error. Would be good to have a table that summarizes the measured absorption for each optic.}

\subsection{Nominal alignment}

Commissioning of the LIGO interferometers yielded an optimum alignment (at which the sensitivity and reliability of the interferometer was maximized) [reasons why?]. This is the nominal alignment of the interferometer. In these alignments, the resonant mode of the interferometer was not centered exactly on the optics. 

Using the Hartmann sensors and the procedure described in the previous section, optical path distortion measurements were made of  multiple optics in O2 and O3 at their nominal alignments. 



Installation and configuration issues prevented measurements of all optics. 
During O2,  the ETM HWS were non-functional but were reconfigured after that observing run and, with the exception of H1-ETMY which remained non-functional, were able to provide optical path distortion measurements for O3.
All 4 ETM optics were replaced after O2.  
All ITM HWS were functional during O2. After O2, H1-ITMX was replaced at LIGO Hanford after a strong point absorber was categorically identified on it. 
All the LIGO test mass optics have unique identifiers, indicated below in parentheses. As a result, reliable absorption data is available on the following optics:



\begin{itemize}
    \item Livingston
    \begin{itemize}
        \item ITMX (ITM-04) [O2/O3]
        \item ITMY (ITM-08) [O2/O3]
        \item ETMX (ETM-10) [O3 only]
        \item ETMY (ETM-15) [O3 only]
    \end{itemize}
    \item Hanford
    \begin{itemize}
        \item ITMX (ITM-03) [O2 only]
        \item ITMX (ITM-07) [O3 only]
        \item ITMY (ITM-11) [O2/O3]
        \item ETMX (ETM-13) [O3 only]
    \end{itemize}
\end{itemize}






Due to the large amount of data, we have opted to  display a subset of the total set of measurements in this section. The first (and most significant) point absorber discovered was on H1-ITMX during O2: a HWS of this is illustrated in Figure \ref{fig:H1ITMX}. For comparison, L1-ITMX, shown in Figure \ref{fig:L1ITMX}, shows no sign of any point absorbers and is consistent with the optical path distortion expected from uniform absorption.

Full data sets can be viewed here [think of something].


\subsection{Highlighting point absorbers with short time scale HWS measurements}


\begin{figure}[h]
  \centering
  \includegraphics[width=\columnwidth]{figures/H1-ITMY_1222497245_1222497366.pdf}
  \caption{H1 ITMY approximately 120s after the interferometer is powered up, showing 6 distinct point absorbers. The origin of the coordinate system has been centered on the main point absorber in this instance. Contours are spaced \SI{1}{\nano\meter} apart. (GPS times of HWS measurements: $t_{\mathrm{REF}} = 1222497245$ [Oct. 02, 2018 06:33:47 UTC], $t_{\mathrm{LIVE}} = 1222497366$).}
  \label{fig:H1ITMY_20s}
  % Figure 1 from P1500260
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=\columnwidth]{figures/H1-ITMY_1222497245_1222498453.pdf}
  \caption{H1 ITMY approximately 20 minutes after the interferometer is powered up, showing diffusion between the point absorbers. The origin of the coordinate system has been centered on the main point absorber in this instance. In this instance, the spread of point absorbers is comparable to the interferometer beam width which, unfortunately, makes it appear similar to uniform absorption.  Contours are spaced \SI{5}{\nano\meter} apart. (GPS times of HWS measurements: $t_{\mathrm{REF}} = 1222497245$ [Oct. 02, 2018 06:33:47 UTC], $t_{\mathrm{LIVE}} = 1222497366$).}
  \label{fig:H1ITMY_1200s}
  % Figure 1 from P1500260
\end{figure}

\textcolor{red}{what do data i want to say about this? A summary of the fitting of the Hartmann sensor measurements? Or simply showing that the points form very quickly. }

Due to the diffusion of heat in glass and the small spatial scale of point absorbers, the thermal lens around a point absorber will form very quickly. Therefore, point absorbers become visible in the Hartmann sensor data after a very short period of time. 
%In contrast, the gradient from uniform absorption takes significantly longer to form. 
Short time scale measurements are very effective for early identification of point absorbers before confusion arises as (a) point absorbers diffuse into uniform absorption and (b) point absorbers diffuse into each other. This is illustrated in Figures \ref{fig:H1ITMY_20s} and \ref{fig:H1ITMY_1200s} which show H1-ITMY after interferometer power-up by approximately 2 minutes and 20 minutes, respectively.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Minimizing uncertainty in absorption  by moving IFO beam}
\begin{figure}[h]
  \centering
  \includegraphics[width=\columnwidth]{figures/H1-ITMY_1234986810_1234987020_H1-ITMY_1235015483_1235015681.png}
  \caption{H1 ITMY approximately 100s after power-up. The IFO beam has been displaced down by approximately \SI{35}{\milli\meter} between these two measurements. Upper panel: $t_{\mathrm{REF}} = 1234986810$ [Feb. 23, 2019 19:53:12 UTC], $t_{\mathrm{LIVE}} = 1234987020$). Lower panel: $t_{\mathrm{REF}} = 1235015483$ [Feb. 24, 2019 03:51:05 UTC], $t_{\mathrm{LIVE}} = 1235015681$).}
  \label{fig:H1ITMY_displacement}
  % Figure 1 from P1500260
\end{figure}

The power absorbed in each point is a function of minimum absorber diameter \Aidan{equivalent spot area (ESA),$a$,} and the local intensity of the IFO beam. 

\begin{equation}
    P_i = a_i\, P_{\mathrm{IFO}}\,I\left(x_i,y_i\right)
\end{equation}

Given that there is some uncertainty in the  position of the HWS coordinate system relative to the IFO beam, there is some uncertainty in the calculated ESA. In fact, given that the uncertainty in the IFO beam center is of the order of \SI{10}{\milli\meter}$\--$\SI{20}{\milli\meter} it will be the dominant source of error in the estimation of the point absorber ESA.


However, it is possible to reduce this error by moving the IFO beam by a known amount, $dx$, and measuring the new absorbed power:

\begin{eqnarray}
    P_i^* & = & a_i\, P_{\mathrm{IFO}}\,I\left(x_i+dx,y_i\right)\\
    & \approx & a_i\, P_{\mathrm{IFO}}\,I\left(x_i,y_i\right)\, \left(1 -\frac{4\, dx\, x_i}{w^2}\right),
\end{eqnarray}

\noindent where the expansion assumes $dx < w$. Taking the relative difference in the absorbed power, we can solve for the position of the point absorber relative to the IFO beam, using:

\begin{equation}
    \frac{\Delta P_i}{P_i} = -\frac{4\, dx\, x_i}{w^2}
    \label{eqn:linear_fit}
\end{equation}

If $dx$ is comparable in size to $w$, it is still possible to use this method by fitting a non-linear function, instead of fitting to Equation \ref{eqn:linear_fit}.


%\textcolor{red}{aLOG 47101}
%\textcolor{red}{Add in uncertainties for beam position and propagate to absorption.}






%Knowing the Gaussian beam profile on each test mass, we use Equation \ref{eqn:MAD} to determine  $D_M$ for each point/ Unfortunately, there is some uncertainty in the exact location of the center of the $I(x,y)$ relative to the center of the HWS coordinate system and this results in  uncertainty in the characterization of $D_M$. 

%The interferometer beam has a Gaussian profile on the optic. If we know the location of the point absorber relative to the center of the Gaussian beam, and hence the local intensity, then it is straightforward to determine the minimum absorber diameter using Equation \ref{eqn:MAD}. Inevitably, there is some uncertainty between the center of the HWS coordinate system and the center of the optic and between the center of the Gaussian beam and the center of the optic.


%\textcolor{magenta}{This paragraph needs some quantization and equations to explain the fitting}.
 %It is possible to minimize the uncertainty by moving the interferometer beam known amounts on the optic. 
 %Given that $D_M$ remains constant, we make multiple measurements of $\Delta P$ for different IFO beam positions (varying the incident intensity on a point absorber) and allowing us to fit for the center of the intensity distribution.

%Therefore, by scanning the  beam around on the test mass (by adjusting the alignment of the Fabry-Perot cavities) we can illuminate point absorbers by varying intensities and explore the distribution and MAD values of those absorbers on the test masses. This is particularly effective if there are multiple point absorbers and the relative change between the two can be observed.

This technique was used to further explore two test masses with multiple absorbers in aLIGO: H1-ITMY, which shows 6 point absorbers and L1-ETMX which shows at least two point absorbers.  Figure \ref{fig:H1ITMY_displacement} shows the   two wavefronts on H1-ITMY taken when the IFO beam has been shifted down between the two.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Summary}

HWS measurements revealed X, Y and Z.







==> modeling.tex <==
\label{sec:modeling}

\Aidan{This section should describe the models we used without discussing the results. It should justify/explain WHY we use particular models. And what the outputs are (and are not). Also, what our ASSUMPTIONS are.}


%\textcolor{red}{Would it make more sense to merge the modeling and results sections? Perhaps discuss the modeling software but, in brief and jump  into the results. RIght now it seems like: we're saying, "in this section, here's a plot from a model of the interferometer behavior and in the following section, here's the same plot but now showing data from the interferometer". Seems silly to separate them without a specific reason (e.g. we can't precisely model the IFO or we don't have data on a specific measurement.}




%\subsection{Discussion of models}
We use  different models of the interferometer, in conjunction with HWS data,  to explain observed, and predict future, interferometer behavior: Finesse \cite{FinesseRef}, MIST \cite{MISTref} and SIS \cite{SIS-T070039}. 



\Aidan{Considering this result, we can see [from some plot that doesn't yet exist] that the 7th order mode is closest to resonance.}


\subsection{Finite-element modeling of test masses}
We use the COMSOL package to produce finite element models of absorption in our test masses. We find that the bulk of the test mass acts a heat bath for energy to dissipate into. Utlimately, power absorbed in the test is radiated to the environment as the average temperature of the optic increases, however, this is on a very long time scale. The thermal gradient is almost totally dependent on thermal conduction. We include radiation in our finite element models for completeness, but it is not necessary for \Aidan{95\%} accuracy. 

This also allows us to ignore boundary conditions (except for the front surface of the test mass). This allows us to model point absorbers as 2D axially symmetric sources of heat. The total optical path distortion, $W_{pt}(r,t)$, is determined. A map of distortion is then produced in Cartesian coordinates using the following summation:

\begin{equation}
    W_{TM}(x,y,t) = a_{0}\,W_{u}(r_0,t) + \sum_{i=1}^{N} a_i\, W_{pt}\,(r_i,t)
\end{equation}

\noindent where $r_{i}$ is given by:

\begin{equation}
    r_{i} = \sqrt{(x-x_i)^2 + (y-y_i)^2}
\end{equation}

\noindent where $[x_i,y_i]$ are the coordinates of the $i-$th point absorber and $[x_0,y_0]$ is the center of the IFO beam for uniform absorption.

The finite element models allow us to apply heat to the 

\Aidan{more words needed here.}




\subsection{Modal models [Finesse, MIST]}

%In this section we explore the interaction of point absorbers with resonant optical cavities to help (a) understand  IFO behavior and (b) predict the negative effect on the sensitivity of aLIGO at full input power. 



Finesse and MIST are steady-state, frequency-domain, multi-spatial mode interferometer simulation tools. At their core, they work by representing the electric fields in an interferometer as a sum of transverse electric modes usually defined in the arm cavity basis. Hence, they are referred to as  {\it modal} expansion simulation tools. They have the advantage that the modal decomposition allows for very fast analysis of interferometer behavior. However, the disadvantage is that a very large number of modes are required to model high-spatial frequency effects, for example, those from a point absorber.


\subsection{FFT-based models [SIS]}

The stationary interferometer simulation (SIS) is a numerical, FFT-based, GW-detector simulation tool. 
It represents the fields in the interferometer as discrete numerical arrays of complex amplitude information and, as such, can calculate fields in optical systems by taking into account realistic details of optical components, like macroscopic shapes, finite-size mirrors and microscopic surface phasemaps. 
Fields are calculated under (quasi-)static or stationary conditions. 

In a typical SIS session, a user would install all mirrors in a setup, defining their properties in the process, lock the resulting cavities and then calculate the resulting field amplitudes at all points in the system. The role of SIS is complimentary to frequency domain (Finesse, MIST) and time domain simulation tools. 

%This is sometimes referred to as a {\it zonal} approach. This naturally encompasses high-spatial frequency effects without having to increase computing capacity. The disadvantages are long run times and ...

%\begin{itemize}
%    \item Stationary interferometer simulation
%    \item easily models highly distorted fields, surface aberrations on optics and finite sized optics
%    \item "For example, “addMirror” is used to install a mirror in the setup, “lock” is used to lock the system and calculate fields and “getField” is used to get field amplitudes" [Hiro]
%    \item https://dcc.ligo.org/LIGO-T070039/public
%\end{itemize}



==> optics_and_pt_absorbers.tex <==
\label{sec:Optics}

%\textcolor{red}{Divergence theorem (Gauss's law) applies. Surface integral vs volume integral of divergence. Provided that the radiation is negligible. SUBSTRATE LENS ALSO EXISTS.}

%\textcolor{blue}{Emphasize the thermal conductivity, $\kappa$ and coefficient of thermal expansion, $\alpha$. Relevant to overall magnitude.}

Given the necessity for high power in the aLIGO arm cavities and the, now confirmed, existence of point absorbers, this section explores the spatial distribution and temporal evolution of thermo-elastic deformation induced by point-like absorption of optical power. 
We also consider the possibility of damage to the optic by examining the corresponding internal stresses.

%\begin{itemize}
%    \item Point absorber becomes a source of heat inside the an optic
%    \item Radiation from surface is small compared to conduction
%    \item Conduction is dominant for most beam sizes
%    \item the heat loss outside the point absorber is only a function of the input power not the point absorber size - even including radiation (as long as it's linear?)
%    \item Hence, outside the region of the point, the heat flow through each hemispherical shell is the same (equal to the inflow of heat).
%    \item Hence, the change in temperature between shells outside the point absorber is the same, regardless of the point absorber size.
%    \item Only differences in temperature distribution will be on the scale of the point absorber.
%\end{itemize}

%\begin{equation}
%    P = -k \, A\, \nabla T
%\end{equation}

\begin{figure}[h]
  \centering
  \includegraphics[width=\columnwidth]{figures/absorption_point.pdf}
  \caption{Power flowing into a point-like region. The radiated power is negligible compared to the conduction. Hence, all power is effectively transferred by conduction. The far-field gradient is only determine by the absorbed power and thermal conductivity.}
  \label{fig:point_absorber}
  % Figure 1 from P1500260
\end{figure}



\subsection{Large scale and small scale deformation and characteristic time scale}

Consider a point-like absorber on the surface of an optic that is exposed to optical power, as illustrated in Figure \ref{fig:point_absorber}. The point-like region absorbs a fraction of the incident power creating a localized temperature gradient. 
To determine the structure (both large scale and small scale) of the temperature gradient, we consider a nested series of hemispheres in a half-infinite piece of glass (ignoring boundary conditions, valid for $w<<a$).

The power conducted through the surface of a hemisphere of radius $r$ is given by:

\begin{equation}
    P_c = \kappa \, \pi\,r\, \Delta T
\end{equation}

\noindent whilst the power lost via radiation through the surface is approximately:

\begin{equation}
    P_r = 4\, \epsilon \, \sigma \, \pi \, r^2 \, \Delta T\, T_{\mathrm{env}}^3
\end{equation}

\noindent and the ratio is:

\begin{equation}
    \frac{2\, \epsilon \, \sigma  \, r \, T_{\mathrm{env}}^3}{ \kappa}
\end{equation}

\noindent where $\epsilon = 0.9$ is the emissivity of fused silica, $\sigma$ is the Stefan-Boltzmann constant, $T_{\mathrm{env}} \approx$ \SI{293}{\kelvin}, and $\kappa =$ \SI{1.38}{\watt\per\meter\per\kelvin}. The ratio of radiated power to conducted increases with radius. However, this ratio is $\le 2\%$ for $r\le$\SI{10}{\milli\meter}. Hence, for  absorbing regions smaller than this radius, we can safely ignore radiation. 

The result is that effectively all the power absorbed within a radius $w$ is conducted through the surface of that hemisphere. That power is then conducted through the surfaces of all successive hemisphere below some reasonable size. The local temperature gradient is given by:

\begin{equation}
    \nabla T = \frac{P}{\kappa\, A}
\end{equation}

The temperature gradient across a given hemisphere depends only on the absorbed power. 
Hence, the temperature gradient of the outer hemispheres do not depend only on the total absorbed power in the point, not the size and shape. 
This is illustrated by a finite-element model of surface deformation from point absorbers of different size but fixed absolute absorbed power, shown in Figure \ref{fig:model_SD}. 
The surface deformation (which depends on the local temperature gradient) varies on the scale of the point absorber size, but is invariant in the large scale.
The conclusion is {\it large scale structure  depends only on absorbed power, not on the point absorber size}. This first key finding is relied upon heavily in the coming analysis.

\begin{figure}[h]
  \centering
  \includegraphics[width=\columnwidth]{figures/uniform_v_pt_abs_cross_section3.pdf}
  \caption{Cross-section of modeled surface deformation from uniform and point absorbers. Incident power = \SI{200}{\kilo\watt} on simulated aLIGO ETM. Uniform absorption (blue) = 200ppb. Point absorber is \SI{38}{\micro\meter} in diameter and 100\% absorbing. The red curve shows the deformation when the absorber is centered on the optic (and then \SI{200}{\kilo\watt} beam). The yellow curve shows the deformation when an identical point absorber is off-center from the beam by \SI{45}{\milli\meter}. \textcolor{red}{FIX THE CAPTION}}
  \label{fig:model_SD}
  % Figure 1 from P1500260
\end{figure}

%\begin{itemize}
%    \item Let us consider the case of a small absorbing region of diameter $2w$. 
%    \item Far field boundary conditions have a certain surface area, $A_F$
%    \item Overall temperature rise is given by far-field
%    \item Assume majority of power lost via thermal conduction.
%    \item Show that power lost from region of spot is negligible
%    \item Hence all power effectively conducted through hemisphere.
%    \item Outside point, hemisphere's only depend on power through the surface,
%    \item thus, outisde the point absorber, the temperature gradient is then agnostic of the size of point absorber size and shape, only depends on input power
%\end{itemize}

%As we study the effects of point absorbers on cavities, we will rely heavily on the conclusion that {\it large scale structure only depends on absorbed power, not on the point absorber size.}


%In the case of a small absorbing region 

%Power radiated from a point is small compared to power conducted. Hence all power lost via conduction around point below a certain size. 


%Diffusion through the optic, coupled with near 100\% loss of power via conduction from the heated region,  effectively masks the large scale temperature gradient from the small scale structure that created it. This implies that the large scale temperature gradient sees no difference between a \SI{20}{\micro\meter} diameter spot that absorbs 100\% of the incident power and a \SI{40}{\micro\meter} diameter spot that absorbs 25\% of the incident power, implying that the  size of the point absorber is less important than the absolute power absorbed.

%In any scenario in which the heat flow out of a region is dominated by conduction and not radiation, we see the following. The region within the mirror that is OUTSIDE the radius of the point absorber sees the same thermal effect regardless of the radius of the point absorber. In other words, outside a radius of \SI{100}{\micro\meter}, the mirror sees the same thermal response from a \SI{100}{\micro\meter} diameter region that absorbs $4\%$ of the incident power and a \SI{20}{\micro\meter} diameter region that absorbs 100\% of the incident power. This will be critical in later sections as the nearly 100\% of the optical field overlaps with regions OUTSIDE the point absorber. 



The characteristic time scale of deformation, however, is a function of the size: for a region, larger than the point absorber, defined by radius, $a$, the characteristic time scale for the temperature gradient (and thus surface deformation) to form between that region and the surrounding environment, is approximated by: 

\begin{equation}
    \tau = \frac{a^2}{3\,D}
\end{equation}

\noindent where $D$ is the thermal diffusivity of the mirror, given by:

\begin{equation}
    D = \frac{\kappa}{\rho\, c}
\end{equation}

\noindent where $\rho$ is the density, $c$ is the specific heat capacity and $\kappa$ is the thermal conductivity, see \cite{sdf}. 

In a more complete analysis, the time-scale for the interaction of surface deformation and a physical effect depends on the spatial weighting function used to characterize that effect. We explore the temporal interaction of the surface deformation with different optical modes in Section \ref{sec:HOM_scattering_tau} to investigate this effect further.


\subsection{Maximum differential stress}

Before considering the optical interaction, it is worth exploring whether a point-like absorber is likely to damage the optic. Let us suppose a flake of aluminum is embedded somewhere within the first few layers of the dielectric coating on an optic.
 In order to determine if this point absorber is likely to cause damage, we model the stress when this point is exposed to high stored power in the interferometer arms using several empirically measured quantities: 

\begin{itemize}
  \item the peak intensity $(I_\mathrm{pk}$): approximately \SI{130}{\watt/\milli\meter^2}, corresponding to a \SI{250}{\kilo\watt} beam  with a Gaussian  radius of \SI{62}{\milli\meter}, 
  \item the absorption $(\epsilon)$ at \SI{1064}{\nano\meter}: approximately 10\%$\--$30\% assuming the material is rough aluminium in nature \cite{ALref},
  \item the absorbed power $(\mathrm{P}_{\mathrm{abs}})$: approximately \SI{17}{\milli\watt} derived from analysis of the Hartmann sensor data.
\end{itemize}

%We assume that the area of the point absorber is concentrated into a circle. The radius, $w$, of this circle is given by:

%\begin{equation}
%    w = \sqrt{\frac{\mathrm{P}_\mathrm{abs}}{\epsilon\,I_\mathrm{pk}\,\pi}}
%    \label{eqn:wsize}
%\end{equation}

%Winkler et al. \cite{Winkler} derived the change in temperature, $\Delta T$, for an absorber of radius, $w$ on the surface of an optic as:

%\begin{equation}
%    \Delta T = \frac{\mathrm{P}_\mathrm{abs}}{2\,\pi\,\kappa\,w},
%    \label{eqn:Winkler}
%\end{equation}

%\noindent where $\kappa$ is the thermal conductivity of the optic. Combining equations \ref{eqn:wsize} and \ref{eqn:Winkler}, we find:

%\begin{equation}
%    \Delta T = \frac{1}{2\,\kappa}\sqrt{\frac{\epsilon\, %\mathrm{P}_\mathrm{abs}\left( I_{\mathrm{pk}} \right)\,I_{\mathrm{pk}}}{\pi}}
%\end{equation}

%Although this yields the change in point absorber temperature in a size-agnostic way, the absorbed power is not independent of the peak intensity (i.e. $P_\mathrm{abs}\propto I_\mathrm{pk}$). 
%Care should be taken when applying this equation to respect that. 
%Assuming room temperature of \SI{20}{\celsius}, the peak temperature ranges from approximately \SI{115}{\celsius} to \SI{185}{\celsius}. As the glass transition temperature for fused silica is $\approx$\SI{1200}{\celsius} \cite{glassT}, we expect no damage from the melting of glass.

The internal stress is examined using a finite element model of a flake of aluminium embedded within the coating of glass, as shown in Figure \ref{fig:embedded_flake}. The constrained flake coupled with differential thermal expansion between it and the fused silica yields a high peak stress. The peak stress observed in the fused silica ($>$\SI{300}{\mega\pascal}) is well in excess of the ultimate tensile thus it is very probable that there will be damage to the coating in this scenario. Indeed, we see evidence for microscopic damage sites on the optics used in O1 and O2.

\begin{figure}[h]
  \centering
  \includegraphics[width=\columnwidth]{figures/flake_aluminium.png}
  \caption{Peak stress in constrained embedded flake of aluminum that absorbs 17mW.}
  \label{fig:embedded_flake}
  % Figure 1 from P1500260
\end{figure}


%The strain, $s$, experienced by the aluminium is estimated by:

%\begin{equation}
%    s = \alpha\, \Delta T, 
%\end{equation}

%\noindent  where $\alpha$ is the coefficient of thermal expansion for aluminium ($=$\SI{23.1E-6}{\per\kelvin}). The expected strain thus ranges from approximately $2.2\times10^{-3}$ to $3.8\times10^{-3}$.

%The stress, $\sigma$, is calculated, in the elastic regime, by 

%\begin{equation}
%    \sigma = E\, s
%\end{equation}

%\noindent where $E$ is the Young's modulus. If the aluminum is embedded in the coating, it is possibly covered by a fused silica layer. So we consider the stress could be distributed in the aluminum and/or fused silica. The Young's modulus of fused silica and aluminium are almost identical, approximately \SI{70}{\giga\pascal}, yielding a stress (assuming the elastic regime), of approximately \SI{160}{\mega\pascal} to \SI{270}{\mega\pascal}. This approaches the tensile strength of aluminium and of fused silica. It is plausible, therefore, that some stress-induced damage may occur due to point absorbers in the surface of the optics.


%\begin{figure}[h]
% \centering
% \includegraphics[width=\columnwidth]{figures/pt_abs_paper_HOM_scattering_plots_COMSOL.pdf}
% \caption{Maximum temperature change and stress in optics vs point absorber diameter for varying levels of absorbed power. The solid purple line is the maximum change in temperature possible for a given spot diameter assuming 100\% absorption and the maximum Fabry-Perot arm power of \SI{750}{\kilo\watt}. The solid purple line in the bottom plot is the corresponding maximum stress for a given spot diameter.}
% \label{fig:maximum_temperature}
  % Figure 1 from P1500260
%\end{figure}






==> otherAWC.tex <==
\label{sec:otherAWC}

\DBrown{Should we cite a bunch of alogs in this section}

One of the goals for observation run 3 was to reach 150kW of circulating power within each of the arm cavities. To achieve this the TCS system is used to compensate for any large scale thermal deformations in the optics so that the mode-matching between the arms and recycling cavities is optimised. This well matched state must be maintained for both a \textit{cold} and \textit{hot} interferometer---cold being the case where the interferometer has been out of a high-power locked state for some time and a low amount of optical is injected, hot being the thermal steady-state when the interferometer is locked and storing significant optical power. During the cold state the TCS system \textit{preloads} the test masses with additional heat from CO2 lasers and ring-heaters to simulate the final hot state of the interferometer. TCS then gradually reduces its actuation as the input power is increased.

At LHO during O3, the point absorbers in ITMY create a significantly stronger thermal lens than ITMX, 800 vs 330~ppb~uD per Watt of optical power stored in the arm cavity. In preparation of this difference the ITMY ring-heater was set to 1.4~W and ITMX ring-heater to 0.5~W to induce an appropriate amount of negative thermal lens to compensate for the additional diffused thermal lensing from the absorbers, as shown in figure~\ref{fig:H1ITMY_1200s}. The large differential ring-heater settings would result in a significantly mismatched interferometer in the cold state, to fix this both CO2 actuators had to be used to thermally preload the test masses, 0.8W for ITMX and 0.9W for ITMY. The ratio is not similar to that of the ring-heater powers, however deviating from this setting introduced significant mismatch in the cold interferometer state and was found to make lock acquisition significantly harder. As the interferometer input power is increased to 35W input, it was found that decreasing CO2-Y to 0W but leaving CO2-X on 0.85W produced the. This results in a  

LLO in O3 however did not require the use of their CO2 actuators for preloading.

Finding the correct balance of cold and hot state TCS settings is a laborious exercise. Both the ring-heaters and CO2 actuators have long time constants, A and B hours respectively. The number of actuator degrees-of-freedom is considerable with four ring-heaters, two CO2 lasers, and the SR3 disk-heater, and with slow actuators it is not possible to quickly explore this parameter space. When locked the TCS settings should be tuned to optimise the lock, when a hot state has been chosen, the cold state preloading must then be updated to match it. This is typically an iterative procedure. 
It was found during the commissioning of LHO for O3 that







% \begin{itemize}
%     \item Differences in LLO vs LHO in ability to power up. Latter has worse point absorber effects and struggled more.
    
%     \item  Some strategies in handling LHO's ITMY and ETMX point absorbers for O3
    
%     \subitem Strategy 1: Adjust estimated existing thermal compensation settings with the intent to mitigate the intermediate spatial frequency effects. 
    
%     \subitem Strategy 2: Moving spot positions on ITM and ETM mirrors. Seemed most effective, reduced OPD, increased circulating powers, more effective on ETMX.
        
%     \subitem Strategy 3: Custom mask for ITMY CO2 actuator. Didn't get to fully implement scheme with RH changes. Although initial attempts at using masks in full lock was helping POP18, arm powers.
    
%     \subitem Strategy 4: SR3 heater increase. At 30W increasing the SR3 heater up to 5W initially gave large improvements. Some of this was attributed to changes in the calibration of DARM at lower frequencies from optical spring effects. SR3 also affected ASC stability at certain heater powers. REFL9 WFS phasing appears to have helped stop a 2min ASC oscillation. RF9 upper and lower have different transmissions from the IFO leading to sideband imbalance, perhaps this is why REFL9 affected by SR3 so much? 
    
%     \subitem Knowledge of PRCL gain dropping helped diagnosing issues of stability from powering up from 20--30W, then ASC tweaks
    
%     \subitem Metrics of improvement: monitor sideband buildups in power recycling cavity, power recycling gain, frequency and intensity noise reduction. Too many metrics to easily make sense of which way to tune TCS
    
%     \subitem Initial TCS attempt to predict 50W thermal load and preload the TCS actuators (Used HWS to characterize ITM and ETM absorption). Gradually offloading as we increase power, worked to some degree. DRMI locking was bad though, perhaps because of CO2 shift causing problematic thermal lens. 
    
%     \subitem Small power steps followed by ASC tunings to regain stability seemed to be the best approach, although time consuming.
    
%     \item Better sensors or metric required for ideal TCS setting. Otherwise TCS tuning can be time inefficient. 
    
% \end{itemize}

==> resonance_summary.tex <==

\subsection{Summary of resonant loss consideration}

The total loss (and reduction of optical gain) is thus a function of several effects, summarized below. All  of these effects must be considered to successfully model the effect of \dfPA{}.

\begin{enumerate}
    \item Amplitude of surface deformation (amplitude of HOM scatter is proportional to amplitude of surface deformation. Power lost is proportional to the amplitude squared).
    \item Spatial location relative to center of TEM00 mode (absorption will vary but the scattering amplitude is strongly dependent on position), as discussed in Section \ref{sec:position_depend}.
    \item Detuned resonant enhancement of HOM which is a function of:
    \begin{enumerate}
      \item The nominal cavity HOM spacing that places some HOM close to resonance, 
      \item Large scale optical surface deformations that detune individual HOM by non-uniform amounts and
      \item Clipping losses in HOM reduce finesse of those modes and increase the detuned resonance of those modes in the arms.
    \end{enumerate}
\end{enumerate}

The cumulative effect of all these elements is illustrated in Figure \ref{}.

%\textcolor{red}{Have a figure here that shows apparent loss as a function of input power for increasingly complex scenarios. A: just scattering out of TEM00 for point at center, B: scattering from resonant cavity, C: scattering with point moved to 20mm from center, D: scenario C with the LHOY arm cavity set-up (which puts TEM70 mode close to center).}
